Spectral independence, coupling with the stationary distribution, and the spectral gap of the Glauber dynamics

We present a new lower bound on the spectral gap of the Glauber dynamics for the Gibbs distribution of a spectrally independent $q$-spin system on a graph $G = (V,E)$ with maximum degree $\Delta$. Notably, for several interesting examples, our bound covers the entire regime of $\Delta$ excluded by arguments based on coupling with the stationary distribution. As concrete applications, by combining our new lower bound with known spectral independence computations and known coupling arguments: (1) We show that for a triangle-free graph $G = (V,E)$ with maximum degree $\Delta \geq 3$, the Glauber dynamics for the uniform distribution on proper $k$-colorings with $k \geq (1.763\dots + \delta)\Delta$ colors has spectral gap $\tilde{\Omega}_{\delta}(|V|^{-1})$. Previously, such a result was known either if the girth of $G$ is at least $5$ [Dyer et.~al, FOCS 2004], or under restrictions on $\Delta$ [Chen et.~al, STOC 2021; Hayes-Vigoda, FOCS 2003]. (2) We show that for a regular graph $G = (V,E)$ with degree $\Delta \geq 3$ and girth at least $6$, and for any $\varepsilon, \delta > 0$, the partition function of the hardcore model with fugacity $\lambda \leq (1-\delta)\lambda_{c}(\Delta)$ may be approximated within a $(1+\varepsilon)$-multiplicative factor in time $\tilde{O}_{\delta}(n^{2}\varepsilon^{-2})$. Previously, such a result was known if the girth is at least $7$ [Efthymiou et.~al, SICOMP 2019]. (3) We show for the binomial random graph $G(n,d/n)$ with $d = O(1)$, with high probability, an approximately uniformly random matching may be sampled in time $O_{d}(n^{2+o(1)})$. This improves the corresponding running time of $\tilde{O}_{d}(n^{3})$ due to [Jerrum-Sinclair, SICOMP 1989; Jerrum, 2003].

==> FPTASunbalancedBIS.tex <==
\section{Bipartite independent set on graph with upper-bounded degree on the left and lower-bounded degree on the right}
\begin{theorem}
Consider bipartite graph $G = G(L,R, E).$ Let $\Delta_L$ be the maximum degree of the vertices in $L$ and $\delta_R$ be the minimum degree of vertices in $R.$ Suppose 
\begin{equation}
    \delta_R \geq 2^{\Delta_L}
\end{equation}
Then the vertices on the left has computational spatial mixing, thus there is a FPTAS for \#BIS (or hardcore-model with fugacity $1$) this model.
\end{theorem}

\begin{lemma}
Easy to see that for vertex $u$ in graph $G'$, the partition function without choosing $u$ is $Z(G'\setminus u, \lambda)$, and the partition function when choosing $u$ is $\lambda Z (G \setminus \mathcal{N}_{G'} [u] , \lambda).$ Thus \[\mu_{G_{i-1}, \lambda}(v_i) = \frac{\lambda Z(G_{i-1} \setminus \mathcal{N}_G[v_i], \lambda)  }{Z (G_{i-1}, \lambda) } = \frac{ \lambda Z (G_i, \lambda) }{Z(G_{i-1}, \lambda) } \]
Let $v_1,\dots, v_n$ be an arbitrary enumeration of vertices in $L.$ Let $G_0 = G$ and $G_i = G_{i-1} \setminus (\{v_i\} \cup \mathcal{N}_{G_{i-1}}(v_i))$ for $i\geq 1.$
Suppose for each $i\geq 1$, we have FPTAS for \[\mu_{G_{i-1}, \lambda}(v_i)= \mathbb{P} [v_i \text{ in independent set sampled according hard-core model with fugacity} \lambda \text{ in } G_{i-1} ]\]
then we have FPTAS for the partition function $Z(G, \lambda)$ of hard-core model on $G.$
\end{lemma}
\begin{proof}
Indeed, we have
\[Z(G, \lambda) = \mu_{G_0, \lambda} (v_1) \mu_{G_1, \lambda} (v_2) \dots \mu_{G_{n-1}, \lambda} (v_n) Z(G_n, \lambda) \]
\end{proof}
\begin{remark}
Compared to Perkins+, this has the advantage of the right-hand degree doesn't have an upper bound ($\Delta_R = \infty$). Disadvantage is the relationship between $\delta_R$ and $\Delta_L$ is much more strict for $\Delta_R \leq ?.$
\end{remark}

==> style.tex <==
\makeatletter %1


% -- Options

\RequirePackage{options}

\options{
	/opts/.new family,
	/opts/colors/.new toggle=true,
	/opts/fonts/.new toggle=true,
	/opts/math/.new toggle=true,
	/opts/theorems/.new toggle=true,
	/opts/macros/.new toggle=true,
	/opts/graphics/.new toggle=true,
	/opts/tools/.new toggle=true,
	/opts/typesetting/.new toggle=true,
	/opts/biblio/.new toggle=true
}
\options{/opts}

\providetoggle{presentation}
\@ifclassloaded{beamer}{\toggletrue{presentation}}{\togglefalse{presentation}}

% -- Packages

\iftoggle{/opts/math}{
	\RequirePackage{amsmath}
	\RequirePackage{amssymb}
	\RequirePackage{bm}
	\RequirePackage{dsfont}
	\RequirePackage{mathtools}
}{}

\iftoggle{/opts/theorems}{
	\RequirePackage{amsthm}
}{}

\iftoggle{/opts/graphics}{
	\RequirePackage{tikz}
	\RequirePackage{tikz-3dplot}
	\RequirePackage{tcolorbox}
	\RequirePackage{pgfplots}
	\RequirePackage{tcolorbox}
	\pgfplotsset{compat=newest}
}{}

\iftoggle{/opts/tools}{
	\RequirePackage[ruled]{algorithm2e}
	\RequirePackage{datatool}
	\RequirePackage[super]{nth}
	\RequirePackage{scalerel}
	\iftoggle{presentation}{}{
		\RequirePackage[shortlabels]{enumitem}
	}
}{}

\iftoggle{/opts/fonts}{
	\iftoggle{presentation}{}{
		\RequirePackage[sc]{mathpazo}
	}
}{}

\iftoggle{/opts/biblio}{
	\iftoggle{presentation}{}{
		\RequirePackage[backend=biber, style=alphabetic, maxbibnames=99, maxcitenames=99, url=false]{biblatex}
	}
}

\iftoggle{/opts/colors}{
	\newcommand{\declarecolor}[2]{\@ifundefined{\string\color@#1}{\definecolor{#1}{RGB}{#2}\expandafter\newcommand\csname #1\endcsname[1]{\textcolor{#1}{##1}}}{}}
	\declarecolor{Black}{0, 0, 0}
	\declarecolor{White}{255, 255, 255}
	\declarecolor{Gray}{127, 127, 127}
	\declarecolor{LightGray}{216, 216, 216}
	\declarecolor{Orange}{237, 125, 49}
	\declarecolor{LightOrange}{251,229, 214}
	\declarecolor{Yellow}{255, 192, 0}
	\declarecolor{LightYellow}{255, 242, 200}
	\declarecolor{Blue}{91, 155, 213}
	\declarecolor{LightBlue}{222, 235, 247}
	\declarecolor{Green}{112, 173, 71}
	\declarecolor{LightGreen}{226, 240, 217}
	\declarecolor{Navy}{68, 114, 196}
	\declarecolor{LightNavy}{218, 227, 243}
	
	\newcommand{\declareperson}[1]{%
		\expandafter\newcommand\csname#1\endcsname[1]{\textcolor{Orange}{#1: ##1}}%
	}
}{}

\iftoggle{/opts/graphics}{
	\RequirePackage{tikzsymbols}
	
	\usetikzlibrary{decorations}
	\usetikzlibrary{decorations.pathreplacing}
	\usetikzlibrary{decorations.markings}
	\usetikzlibrary{fit}
	\usetikzlibrary{intersections}
	\usetikzlibrary{matrix}
	\usetikzlibrary{overlay-beamer-styles}
	\usetikzlibrary{patterns}
	\usetikzlibrary{shapes}
	\usetikzlibrary{tikzmark}
	\usetikzlibrary{hobby}
	
	\usepgflibrary{arrows.meta}
	
	\tcbuselibrary{skins}
	\tcbuselibrary{raster}
	
	\usepgfplotslibrary{patchplots}
		
	\pgfdeclarelayer{background}
	\pgfdeclarelayer{foreground}
	\pgfsetlayers{background,main,foreground}
	\tikzstyle{na}=[baseline=-0.5ex]
	\tikzset{onslide/.code args={<#1>#2}{%
	  \only<#1>{\pgfkeysalso{#2}}
	}}
	\tikzset{temporal/.code args={<#1>#2#3#4}{%
	  \temporal<#1>{\pgfkeysalso{#2}}{\pgfkeysalso{#3}}{\pgfkeysalso{#4}}
	}}
		
	\pgfplotsset{colormap={WhiteOrange}{
		color=(White)
		color=(Orange)
	}}
	\pgfplotsset{colormap={NavyOrange}{
		color=(LightNavy)
		color=(Orange)
	}}
	\pgfplotsset{colormap={WhiteNavy}{
		color=(White)
		color=(Navy)
	}}
	\pgfplotsset{colormap={WhiteBlack}{
		color=(White)
		color=(Black)
	}}
		
	\newcommand*{\Pic}[2][]{\begin{tikzpicture}\pic[#1]{#2};\end{tikzpicture}}
	\newcommand*{\sPic}[2]{\scalebox{#1}{\Pic{#2}}}
	\newcommand*{\cPic}[2][]{\begin{center}\Pic[#1]{#2}\end{center}}
	
	\newcommand{\rounded}[2][0.7ex]{%
		\begin{tikzpicture}
			\node[inner sep=0ex, draw=White, line width=0ex, opacity=0.] (a) {#2};
			\clip[rounded corners=#1] (a.south west) rectangle (a.north east);
			\node[inner sep=0ex] (a) {#2};
		\end{tikzpicture}%
	}
	
	\newcommand*{\tnode}[2]{\tikzmarknode{#1}{#2}}
}{}

\iftoggle{/opts/typesetting}{
	\iftoggle{presentation}{
	}{
		\RequirePackage{microtype}
		\RequirePackage[noblocks]{authblk}
		\RequirePackage{parskip}
		\RequirePackage{fullpage}
	}
	\RequirePackage{hyperref}
	\RequirePackage[capitalize, nameinlink]{cleveref}
	
	\iftoggle{/opts/colors}{
		\hypersetup{
			colorlinks=true,
			pdfpagemode=UseNone,
			citecolor=Green,
			linkcolor=Navy,
			urlcolor=Black
		}
	}{}
}{}

\iftoggle{/opts/theorems}{
	\iftoggle{presentation}{}{
		\theoremstyle{plain}
		\newtheorem{theorem}{Theorem}
		\newtheorem{lemma}[theorem]{Lemma}
		\newtheorem{corollary}[theorem]{Corollary}
		\newtheorem{proposition}[theorem]{Proposition}
		\newtheorem{fact}[theorem]{Fact}
		\newtheorem{conjecture}[theorem]{Conjecture}
		\newtheorem*{conjecture*}{Conjecture}
		
		\theoremstyle{definition}
		\newtheorem{definition}[theorem]{Definition}
		
		\theoremstyle{remark}
		\newtheorem{remark}[theorem]{Remark}
		\newtheorem{example}[theorem]{Example}
		\newtheorem{claim}[theorem]{Claim}
	}
}{}

\iftoggle{/opts/macros}{
	\providecommand{\given}{}
	\newcommand\GivenSymbol[1][]{%
		\nonscript\:#1\vert%
		\allowbreak%
		\nonscript\:%
		\mathopen{}%
	}
	\providecommand{\mid}{}
	\newcommand\MidSymbol[1][]{%
		\nonscript\:#1\|%
		\allowbreak%
		\nonscript\:%
		\mathopen{}%
	}
	\newcommand{\declaredelims}[3]{%
		\expandafter\DeclarePairedDelimiterX\csname#1\endcsname[1]{#2}{#3}{\renewcommand\given{\GivenSymbol[\delimsize]}\renewcommand\mid{\MidSymbol[\delimsize]}##1}%
	}
	
	\declaredelims{set}\{\}
	\declaredelims{card}\lvert\rvert
	\declaredelims{abs}\lvert\rvert
	\declaredelims{norm}\lVert\rVert
	\declaredelims{dotp}\langle\rangle
	\declaredelims{tuple}\lparen\rparen
	\declaredelims{parens}\lparen\rparen
	\declaredelims{bracks}\lbrack\rbrack
	
	\newcommand{\declarenameddelims}[4]{%
		\expandafter\DeclarePairedDelimiterXPP\csname#1\endcsname[1]{#2}{#3}{#4}{}{\renewcommand\given{\GivenSymbol[\delimsize]}\renewcommand\mid{\MidSymbol[\delimsize]}##1}%
		\expandafter\DeclarePairedDelimiterXPP\csname#1X\endcsname[2]{#2_{##1}}{#3}{#4}{}{\renewcommand\given{\GivenSymbol[\delimsize]}\renewcommand\mid{\MidSymbol[\delimsize]}##2}%
	}
	
	
	\let\P\relax
	\declarenameddelims{P}{\mathbb{P}}\lbrack\rbrack
	\declarenameddelims{Ex}{\mathbb{E}}\lbrack\rbrack
	
	\newcommand*{\eval}[1]{\left.#1\right\rvert}
	
	\iftoggle{presentation}{%
		\newcommand*{\mathdouble}[1]{\mathds{#1}}%
	}{%
		\newcommand*{\mathdouble}[1]{\mathbb{#1}}%
	}
	
	\let\Q\relax
	\newcommand*{\Q}{{\mathdouble{Q}}}
	\let\N\relax
	\newcommand*{\N}{{\mathdouble{N}}}
	\let\Z\relax
	\newcommand*{\Z}{{\mathdouble{Z}}}
	\let\R\relax
	\newcommand*{\R}{{\mathdouble{R}}}
	\let\C\relax
	\newcommand*{\C}{{\mathdouble{C}}}
	\let\1\relax
	\newcommand*{\1}{{\mathds{1}}}
	\let\l\relax
	\newcommand*{\l}{{\ell}}
	
	\let\poly\relax
	\DeclareMathOperator{\poly}{poly}
	\DeclareMathOperator{\supp}{supp}
	\DeclareMathOperator{\conv}{conv}
	\DeclareMathOperator{\rank}{rank}
	\let\Im\relax
	\DeclareMathOperator{\Im}{Im}
	\let\Re\relax
	\DeclareMathOperator{\Re}{Re}
}{}
\makeatother

